Towards Complex Dynamic Physics System Simulation with Graph Neural ODEs

The great learning ability of deep learning models facilitates us to comprehend the real physical world, making learning to simulate complicated particle systems a promising endeavour. However, the complex laws of the physical world pose significant challenges to the learning based simulations, such as the varying spatial dependencies between interacting particles and varying temporal dependencies between particle system states in different time stamps, which dominate particles' interacting behaviour and the physical systems' evolution patterns. Existing learning based simulation methods fail to fully account for the complexities, making them unable to yield satisfactory simulations. To better comprehend the complex physical laws, this paper proposes a novel learning based simulation model- Graph Networks with Spatial-Temporal neural Ordinary Equations (GNSTODE)- that characterizes the varying spatial and temporal dependencies in particle systems using a united end-to-end framework. Through training with real-world particle-particle interaction observations, GNSTODE is able to simulate any possible particle systems with high precisions. We empirically evaluate GNSTODE's simulation performance on two real-world particle systems, Gravity and Coulomb, with varying levels of spatial and temporal dependencies. The results show that the proposed GNSTODE yields significantly better simulations than state-of-the-art learning based simulation methods, which proves that GNSTODE can serve as an effective solution to particle simulations in real-world application.

==> 8_discuss_and_future_work.tex <==
The actual physical world's changes are significantly more complex than we believe. Although our model provides a solution for the dimensions of space and time, it has a long way to go before it can comprehend the laws of the real world. In addition to the three primary jobs, we can envision a series of tasks, such as environment interaction (e.g. boundary difficulties) and the interaction of increasingly complicated substances with various qualities, which must be investigated. In addition to these issues with the Lagrangian method, the Euler-based model will also encounter comparable difficulties. Therefore, a great deal of actual work for AI in science must be urgently identified and investigated.
